Local stability of McKean-Vlasov equations arising from heterogeneous Gibbs systems using limit of relative entropies

A family of heterogeneous mean-field systems with jumps is analyzed. These systems are constructed as a Gibbs measure on block graphs. When the total number of particles goes to infinity, a law of large numbers is shown to hold in a multi-class context resulting in the weak convergence of the empirical vector towards the solution of a McKean-Vlasov system of equations. We then investigate the local stability of the limiting McKean-Vlasov system through the construction of a local Lyapunov function. We first compute the limit of adequately scaled relative entropy functions associated with the explicit stationary distribution of the N-particles system. Using a Laplace principle for empirical vectors we show that the limit takes an explicit form. Then we demonstrate that this limit satisfies a descent property which, combined with some mild assumptions shows that it is indeed a local Lyapunov function.

==> babelbst.tex <==
%%
%% This is file `merlin.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from merlin.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
%\ifcase\language \input{frenbst} \or \input{frenbst}
%\else \input{frenbst} \fi
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{r\'edacteurs}        \def\bbleds{r\'ed.}
\def\bbleditor{r\'edacteur}          \def\bbled{r\'ed.}
\def\bbledby{edit\'e par}
\def\bbledition{edition}        \def\bbledn{ed}
\def\bblvolume{tome}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n$^\mathrm{o}$}
\def\bblin{dans}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Rapport technique}
\def\bbltechrep{Rap. Tech.}
\def\bblmthesis{Th\`ese de ma\^itre}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1ere}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\`eme}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\`eme}
\def\bblfourth{Quatri\`eme}          \def\bblfourtho{4\`eme}
\def\bblfifth{Cinqui\`eme}            \def\bblfiftho{5\`eme}
\def\bblst{$^{\mbox{\scriptsize \`ere}}$}  
\def\bblnd{$^{\mbox{\scriptsize \`eme}}$}  
\def\bblrd{$^{\mbox{\scriptsize \`eme}}$}
\def\bblth{$^{\mbox{\scriptsize \`eme}}$}
\def\bbljan{janvier}  \def\bblfeb{f\'evrier}  \def\bblmar{mars}
\def\bblapr{avril}    \def\bblmay{mai}       \def\bbljun{juin}
\def\bbljul{juillet}     \def\bblaug{ao\^ut}    \def\bblsep{septembre}
\def\bbloct{octobre}  \def\bblnov{novembre}  \def\bbldec{d\'ecembre}
\endinput
%%
%% End of file `merlin.tex'.

